Adapting Self-Supervised Representations to Multi-Domain Setups

Current state-of-the-art self-supervised approaches, are effective when trained on individual domains but show limited generalization on unseen domains. We observe that these models poorly generalize even when trained on a mixture of domains, making them unsuitable to be deployed under diverse real-world setups. We therefore propose a general-purpose, lightweight Domain Disentanglement Module (DDM) that can be plugged into any self-supervised encoder to effectively perform representation learning on multiple, diverse domains with or without shared classes. During pre-training according to a self-supervised loss, DDM enforces a disentanglement in the representation space by splitting it into a domain-variant and a domain-invariant portion. When domain labels are not available, DDM uses a robust clustering approach to discover pseudo-domains. We show that pre-training with DDM can show up to 3.5% improvement in linear probing accuracy on state-of-the-art self-supervised models including SimCLR, MoCo, BYOL, DINO, SimSiam and Barlow Twins on multi-domain benchmarks including PACS, DomainNet and WILDS. Models trained with DDM show significantly improved generalization (7.4%) to unseen domains compared to baselines. Therefore, DDM can efficiently adapt self-supervised encoders to provide high-quality, generalizable representations for diverse multi-domain data.

==> tables_and_figures/resource_usage.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.5\textwidth}{!}
{
    \begin{tabular}{c|c|c}
    \toprule
         \textbf{Resource} & \textbf{Single-Domain SimCLR} & \textbf{MDSSL}  \\
    \midrule
    \midrule
         Training Time (hours) & 42.41 & \textbf{34.95} (-17.59\%) \\
         Disk Memory (MB) & 968 & \textbf{242} (-75\%) \\
         Compute (GPUs) & 3 & \textbf{1} (-66.66\%) \\
    \bottomrule
    \end{tabular}
}
\caption{Resource utilization of SimCLR and MDSSL when trained on CIFAR-10, STL-10 and CIFAR-100}
    \label{tab:resource_usage}
\end{table}
